General Object Foundation Model for Images and Videos at Scale

We present GLEE in this work, an object-level foundation model for locating and identifying objects in images and videos. Through a unified framework, GLEE accomplishes detection, segmentation, tracking, grounding, and identification of arbitrary objects in the open world scenario for various object perception tasks. Adopting a cohesive learning strategy, GLEE acquires knowledge from diverse data sources with varying supervision levels to formulate general object representations, excelling in zero-shot transfer to new data and tasks. Specifically, we employ an image encoder, text encoder, and visual prompter to handle multi-modal inputs, enabling to simultaneously solve various object-centric downstream tasks while maintaining state-of-the-art performance. Demonstrated through extensive training on over five million images from diverse benchmarks, GLEE exhibits remarkable versatility and improved generalization performance, efficiently tackling downstream tasks without the need for task-specific adaptation. By integrating large volumes of automatically labeled data, we further enhance its zero-shot generalization capabilities. Additionally, GLEE is capable of being integrated into Large Language Models, serving as a foundational model to provide universal object-level information for multi-modal tasks. We hope that the versatility and universality of our method will mark a significant step in the development of efficient visual foundation models for AGI systems. The model and code will be released at https://glee-vision.github.io .

==> table/LISA.tex <==
\begin{table}
\renewcommand\arraystretch{0.9}
    \small 
    \centering
    
   \resizebox{\columnwidth}{!}{
    \begin{tabular}{*4{c|ccc|ccc|cc}}
    \toprule
  LISA   & Ref(val) & Ref(testA)  & Ref(testB)   & Ref+(val) & Ref+(testA)  & Ref+(testB)   & Refg(val) & Refg(test) \\
    \midrule
    w/o \methodNAME & 76.95 & 79.25  &73.78  &67.65  &72.42  &61.38   &70.83 &71.96 \\
    w/\methodNAME  &76.35 &78.24  &73.81  &67.31  &71.25  &62.33  &71.56  &72.37  \\
    \bottomrule
    \end{tabular}}
    \vspace{-2ex}
    \caption{ 
The performance comparison of replacing SAM with \methodNAME in LISA, where Ref, Ref+, and Refg correspond to results on RefCOCO, RefCOCO+, and RefCOCOg, respectively.
\methodNAME achieves the same effectiveness as SAM in extracting objects.
}
    \label{table:LISA}
    \vspace{-2ex}
\end{table}


==> table/burst.tex <==
\begin{table}[!ht]
\centering
\resizebox{1.0\linewidth}{!}{
\setlength{\tabcolsep}{2pt}
\begin{tabular}{lcccccc}
\toprule 
\multirow{2}{*}{Method}   & \multicolumn{2}{c}{ALL}   & \multicolumn{2}{c}{Common}    & \multicolumn{2}{c}{Uncommon} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
&$\rm HOTA$    &$\rm mAP$ &$\rm HOTA$    &$\rm mAP$  &$\rm HOTA$    &$\rm mAP$  \\

\midrule
STCN Tracker~\cite{burst}     & 5.5 & 0.9 &17.5  & 0.7   &2.5  &0.6  \\
Box Tracker~\cite{burst}      & 8.2  &1.4  &27.0  &3.0   &3.6   &0.9\\
\methodNAME-Lite   &22.6  &12.6  &36.4  &18.9   &19.1   &11.0 \\
\methodNAME-Plus   &26.9  &17.2  &38.8  &23.7  &23.9   &15.5   \\
\methodNAME-Pro    &31.2   &19.2   &48.7   &24.8   &26.9  &17.7\\
\bottomrule

\end{tabular}}


\caption{
Performance comparison of our \methodNAME on large vocabulary multi-object tracking and segmentation benchmark BURST~\cite{burst}.)
}
\label{table:vis_results}
\end{table}


==> table/data_scale_ablation.tex <==

\begin{table}[t]
\centering
\setlength{\tabcolsep}{3.1pt}
\small


\begin{tabular}{r|cccccccc}
\toprule
Data&& TAO && BURST && OVIS && {YTVIS} \\
\cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9}
size && $\rm TETA$ && $\rm HOTA$ &&$\rm mAP$ && mAP \\
\midrule
10\% &&  45.6 && 26.0 && 34.1 && 65.0   \\ 
20\% &&  45.2 && 29.5 && 35.0 && 66.5    \\ 
50\% &&  45.5 && 30.6 && 35.9 && 67.0 \\ 
100\% &&   \textbf{47.2} && \textbf{31.2} && \textbf{38.7} && \textbf{67.4}  \\ 
\bottomrule
\end{tabular}

\caption{\textbf{Data scaling.} Zero-shot performance on TAO, BURST, OVIS, YTVIS19.}
\label{tab:ablation_data_scaling}
    \vspace{-2ex}
\end{table}

==> table/tao.tex <==

\begin{table}[t]
\footnotesize
\centering

\resizebox{0.72\linewidth}{!}{
\begin{tabular}{l|cccc}
\toprule
Method                            &   TETA   & LocA  & AssocA & ClsA  \\ \midrule 
SORT-TAO~\cite{tao}       & 24.8 & 48.1 & 14.3  & 12.1 \\
Tracktor~\cite{bergmann2019tracking}                          & 24.2  & 47.4 & 13.0  & 12.1 \\
DeepSORT~\cite{wojke2017simple}                         & 26.0  & 48.4 & 17.5  & 12.1 \\
AOA~\cite{du2021aoa}                               & 25.3  & 23.4 & 30.6  & {21.9} \\
Tracktor++~\cite{tao}                        & 28.0  & 49.0 & 22.8  & 12.1 \\
QDTrack~\cite{QDTrack}                       & 30.0  & 50.5 & 27.4  & 12.1 \\
TETer~\cite{li2022tracking}                            & 33.3  & {51.6} & 35.0  & 13.2 \\ \midrule
OVTrack$\dagger$  ~\cite{li2023ovtrack}        & 34.7  & 49.3 & {36.7}  & 18.1 \\
\methodNAME-Lite$\dagger$  &40.1  &56.3  &39.9  &24.1  \\
\methodNAME-Plus$\dagger$  &41.5  &52.9  &40.9  &\textbf{30.8}  \\
\methodNAME-Pro$\dagger$  &\textbf{47.2}  &\textbf{66.2}  &\textbf{46.2}  &29.1  \\
\bottomrule
\end{tabular}}
% \vspace{-3mm}
\label{comparison:teta}
\caption{\textbf{Zero-shot transfer to large-vocabulary MOT task TAO~\cite{tao}.} We compare to existing trackers on the TAO~\cite{tao} validation. Benchmark results are taken from~\cite{li2022tracking}. All competing methods use ResNet101~\cite{resnet} except AOA~\cite{du2021aoa}, OVTrack uses ResNet50 as backbone. $\dagger$ does not use videos for training.}\vspace{-2mm}
\end{table}





==> table/zeroshot_video.tex <==
\begin{table*}[ht]
    \centering
    \begin{minipage}{.32\textwidth}
        \centering
            \resizebox{1.0\linewidth}{!}{
            \begin{tabular}{l|cccc}
            \toprule
            Method                            &   TETA   & LocA  & AssocA & ClsA  \\ \midrule 
            % SORT-TAO~\cite{tao}       & 24.8 & 48.1 & 14.3  & 12.1 \\
            Tracktor~\cite{bergmann2019tracking}                          & 24.2  & 47.4 & 13.0  & 12.1 \\
            DeepSORT~\cite{wojke2017simple}                         & 26.0  & 48.4 & 17.5  & 12.1 \\
            % AOA~\cite{du2021aoa}                               & 25.3  & 23.4 & 30.6  & {21.9} \\
            Tracktor++~\cite{tao}                        & 28.0  & 49.0 & 22.8  & 12.1 \\
            QDTrack~\cite{QDTrack}                       & 30.0  & 50.5 & 27.4  & 12.1 \\
            TETer~\cite{li2022tracking}                            & 33.3  & {51.6} & 35.0  & 13.2 \\ \midrule
            OVTrack$\dagger$  ~\cite{li2023ovtrack}        & 34.7  & 49.3 & {36.7}  & 18.1 \\
            \methodNAME-Lite$\dagger$  &40.1  &56.3  &39.9  &24.1  \\
            \methodNAME-Plus$\dagger$  &41.5  &52.9  &40.9  &\textbf{30.8}  \\
            \methodNAME-Pro$\dagger$  &\textbf{47.2}  &\textbf{66.2}  &\textbf{46.2}  &29.1  \\
            \bottomrule
            \end{tabular}
            }
        \caption{\textbf{Zero-shot transfer to large-vocabulary MOT task TAO~\cite{tao}.} We compare to existing trackers on the TAO~\cite{tao} validation. $\dagger$ does not use videos for training.}
        \label{tab:table1}
    \end{minipage}%
    \hfill
    \begin{minipage}{.39\textwidth}
        \centering
        \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{lcccccc}
            \toprule 
            \multirow{2}{*}{Method}   & \multicolumn{2}{c}{ALL}   & \multicolumn{2}{c}{Common}    & \multicolumn{2}{c}{Uncommon} \\
            \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
            &$\rm HOTA$    &$\rm mAP$ &$\rm HOTA$    &$\rm mAP$  &$\rm HOTA$    &$\rm mAP$  \\
            
            \midrule
            STCN Tracker~\cite{burst}     & 5.5 & 0.9 &17.5  & 0.7   &2.5  &0.6  \\
            Box Tracker~\cite{burst}      & 8.2  &1.4  &27.0  &3.0   &3.6   &0.9\\
            \methodNAME-Lite   &22.6  &12.6  &36.4  &18.9   &19.1   &11.0 \\
            \methodNAME-Plus   &26.9  &17.2  &38.8  &23.7  &23.9   &15.5   \\
            \methodNAME-Pro    &31.2   &19.2   &48.7   &24.8   &26.9  &17.7\\
            \bottomrule
            
            \end{tabular}
            }
        \caption{Zero-shot transfer performance comparison of our \methodNAME on large vocabulary multi-object tracking and segmentation benchmark BURST~\cite{burst}. Two baseline trackers employ Mask-RCNN trained on LVIS~\cite{lvis} as the detector. Evaluation metrics are reported separately for ‘common’, ‘uncommon’ and ‘all’ classes. }
        \label{tab:table2}
    \end{minipage}
    \hfill
    \begin{minipage}{.25\textwidth}
        \centering
                \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{lccc}
            \toprule 
            % \multirow{2}{*}{Method}   & \multicolumn{2}{c}{ALL}   & \multicolumn{2}{c}{Common}    & \multicolumn{2}{c}{Uncommon} \\
            \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
           Method &$\rm AP$  &$\rm AP_b$    &$\rm AB_n$  \\
            
            \midrule
            Detic [57]-SORT [8]    & 12.8 & 21.1 &6.6      \\
            Detic [57]-XMem [13]   & 16.3  &24.1 &10.6  \\
            OV2Seg-R50    &14.2 &17.2 &11.9\\
            OV2Seg-B       &21.1 &27.5 &16.3 \\
            \methodNAME-Lite  &19.6 &22.1 &17.7 \\
            \methodNAME-Plus   &30.3 &31.6 &29.3  \\
            \methodNAME-Pro      \\
            \bottomrule
            
            \end{tabular}
            }
        \caption{The performance comparison on LV-VIS validation set. The AP, APb, and APn mean the average precision of
        overall categories, base categories, and novel categories. }
        \label{tab:table3}
    \end{minipage}
\end{table*}

